DUET: 2D Structured and Approximately Equivariant Representations

Multiview Self-Supervised Learning (MSSL) is based on learning invariances with respect to a set of input transformations. However, invariance partially or totally removes transformation-related information from the representations, which might harm performance for specific downstream tasks that require such information. We propose 2D strUctured and EquivarianT representations (coined DUET), which are 2d representations organized in a matrix structure, and equivariant with respect to transformations acting on the input data. DUET representations maintain information about an input transformation, while remaining semantically expressive. Compared to SimCLR (Chen et al., 2020) (unstructured and invariant) and ESSL (Dangovski et al., 2022) (unstructured and equivariant), the structured and equivariant nature of DUET representations enables controlled generation with lower reconstruction error, while controllability is not possible with SimCLR or ESSL. DUET also achieves higher accuracy for several discriminative tasks, and improves transfer learning.

==> sections/introduction.tex <==
\section{Introduction}

% Learn from unlabelled data. 
% Main strategies:
% * Multiview SSL: learn invariances that the designer thinks are not aligned with the downstream performance. Good for classification (some), but not good for other cls tasks.
%     - Look for references for SSL + Gen
%     - Look for references for SSL + Segmentation, ObjDet

% * Equivariance is helpful 

% SSL quick overview. Main advantages: \\
%   - generic features \\
%   - massive amounts of data \\
%   - multimodal
  
  
% Unsupervised learning, or learning from unlabelled data, enables using large scale datasets with no annotation effort. One important application of unsupervised learning is representation learning, where the goal is to obtain compressed representations of the data that contain all the relevant semantic aspects. The fundamental problem in representation learning is to decide what information is discarded or preserved to construct useful representations.

The field of representation learning has evolved at a fast pace in recent years, partially due to the popularity of Multiview Self-Supervised Learning (MSSL). The main idea of MSSL is to learn representations by comparing differently transformed versions (views) of the data. The underlying hypothesis is that the transformations applied introduce task-irrelevant information, thus multiple views of the same image should yield similar representations that only contain task-relevant information. In other words, the representations become invariant to the input transformations applied. Such an idea is often put into practice with variants of the InfoNCE loss \cite{cpc}, popularly named as contrastive MSSL approaches \cite{simclr, moco, swav}, where views of the same image are contrasted with views of other images. Alternatively, other works have explored MSSL from a non-contrastive perspective, by only comparing pairs of the same image \cite{byol, btwins}. In these works, additional regularization is required, such as encoding one of the views with a shifted and frozen version of the main encoder. \todo{Do we need to mention contrastive and non-contrastive?}
 
The end goal of MSSL is to learn generic representations useful for \textit{any} downstream task. Thus, the input transformations should be diverse enough to generate informative views, and also carefully selected so that task-relevant information is preserved at the representation level. However, both requirements are impossible to satisfy in practice, and one can always find a downstream task for which the chosen transformations are ineffective. For example, MSSL representations learnt using color transformations will fail for the downstream task of predicting fruit ripeness (color information is required). Moreover, multiple transformations are typically applied at once (transformation stacks) which increases the number of ill-posed downstream tasks. Beyond classification or regression counterexamples, representations learnt via MSSL remove too much detail for other tasks to be successful, such as generation or segmentation \cite{hybgencon}. 
%Summarizing, MSSL representations are tailored to work for tasks that do not require information related to the input transformations used.
%Many works have explored the most suitable transformations stacks for both supervised learning and MSSL \cite{fastaugment, autoaugment, randaugment, populationaugment}. However, the outcome of these works is still unclear \cite{arno_aug}.

One strategy to enhance task-relevant information in MSSL is to encourage discarding task-irrelevant information. For example, with an explicit loss \cite{SSL_MV} or relaxing the invariance constraint by allowing a residual when comparing representations \cite{residualssl}. However, the underlying problem of knowing which invariances to learn is still present. Instead of discarding information, equivariant models preserve both task-relevant and task-irrelevant information in the representations \cite{gcnn, arblie, qtae, offseteq, tvae}. These models exploit symmetries in the data that can be expressed as algebraic groups. Note that one can still achieve the desired invariance by training a final layer on top of the equivariant representations. Furthermore, equivariant models show improved robustness both for supervised learning (SL) \cite{gcnn, sesn} and MSSL \cite{essl, hssl}. 
However, equivariant models have some drawbacks: (1) they are designed for finite groups, where the number of group elements is usually small (\eg $90^{\circ}$ rotations), (2) suppose an increase in compute time and memory and (3) to the best of our knowledge do not perform well for non-exact algebraic groups (\eg color-related transformations).% or compositions of groups.

%and have been, etc. Not clear if features specific to each transformation are encouraged to learn, or just the augmentation information is transferred to the representation. \textit{Extreme case example, one float regresses the augmentation parameter and the remaining of the features stay the same. }
%Equivariant neural networks \cite{GCNN, SESN, etc} learn structured representations by using transformed versions of CNN filters, yielding representations specific to each group element. Equivariant models have some drawbacks: (1) they are designed for finite groups, where the number of group elements is usually small (\eg $90^{\circ}$ rotations), (2) suppose an increase in compute time and memory and (3) to the best of our knowledge do not perform well for color-related transformations or compositions of more than 2 groups.

We propose to model the joint distribution over \textit{content} ($\sC$) and \textit{group} ($\sG$) element using MSSL.
The group element defines the input transformation applied, while the content includes all the information in the image that is invariant to the group actions. Our formulation allows a natural marginalization of content and group, which can be maximized separately. We maximize the content marginal by maximizing agreement between two views of the same image as in \cite{simclr}. The group marginal is matched to a known prior by means of Jensen-Shannon Divergence. The resulting representation is structured in terms of group elements.
\method addresses the drawbacks mentioned for equivariant networks: (1) naturally handles finite and continuous groups, (2) does not increase the compute time and (3) naturally handles learning  jointly for an arbitrary number of groups. Additionally, we show that \method representations are explicitly equivariant and can be transformed analytically in feature space, as opposed to \cite{essl, augself}.

Representations learnt with \method improve top-1 test performance compared to a SimCLR \cite{simclr} baseline. We also improve performance for all group-specific augmentations tested, and we compare favorably with NPTN \cite{nptn} and ESSL \cite{essl}. We additionally show that \method representations drastically improve generative performance (up to $3\times$ better reconstruction error than SimCLR representations) and better downstream performance to a large set of classification tasks. Finally, \method allows direct recovery of the input transformation parameter of an arbitrary image, without requiring any specialized regression head or classifier (as in \cite{essl, augself}), which improves interpretability.
% One key aspect of equivariant networks is that they learn a representation \textit{per finite group element}. Therefore, an image is represented by the aggregation of the representations for all group elements. Inspired by this over-complete aspect of equivariant representations we propose \method, a new method to learn an over-complete representation that addresses the drawbacks mentioned for equivariant networks: (1) naturally handles continuous groups, (2) does not increase the compute time and (3) we show theoretically and empirically how structure is learnt jointly for an arbitrary number of groups. \method's core idea is to treat the latent representation of our SSL backbone as a joint probability distribution over \textit{content} ($\sC$) and \textit{group} ($\sG$). The group defines the input transformation applied, while the content includes all the  information of the image that is invariant to the group actions. Our formulation allows an easy marginalization of content and group, which can be maximized separately. We maximize the content marginal distributions between two views using a contrastive loss as in \cite{simclr}, and to match the marginal group distribution to a Gaussian prior. The resulting joint representation learnt is structured both in terms of content (features describing the images) and group elements. 
Summarizing, our main contributions are \todo{Update}:
\begin{itemize}
    \item \method, a method to learn the structured representations for arbitrary (continuous and finite) groups with no computational overhead. Our approach also performs well for parameterized transformations that do not satisfy all algebraic group axioms, making it widely applicable to all transformations used in MSSL.
    \item Extensive experiments on MNIST, CIFAR10, CIFAR100 and TinyImageNet; showing the benefits of using \method representations for classification and generation in the MSSL setting.
    \item A theoretical formulation and empirical validation of equivariance learnt using \method.
    % \item We further show how equivariance can be exploited for conditioned image generation.
    % \item Our method also strongly improves the efficacy of self-supervised features for generative purposes. We show that the reconstruction error is drastically reduced with respect to SimCLR feature. Moreover, we show reconstruction can be easily controlled thanks to the equivariance properties of our features.
    % \item Allows 0-shot regression of the augmentation parameters applied on a test image! 
    % \item An analysis on the coupling of different augmentations, hinting which augmentations are actually useful.
\end{itemize}

% Ideas:
% \begin{itemize}
%     \item Can we beat ESSL for gray-scale, blur, flip, etc.? Running in \texttt{moedec3k-A0fli}.
%     \item Implement ESSL as second baseline! Show MSE and parameter regression performance.
%     \item Check if we can regress parameters for joint groups.
% \end{itemize}



==> sections/introduction2.tex <==
\section{Introduction}

% Learn from unlabelled data. 
% Main strategies:
% * Multiview SSL: learn invariances that the designer thinks are not aligned with the downstream performance. Good for classification (some), but not good for other cls tasks.
%     - Look for references for SSL + Gen
%     - Look for references for SSL + Segmentation, ObjDet

% * Equivariance is helpful 

% SSL quick overview. Main advantages: \\
%   - generic features \\
%   - massive amounts of data \\
%   - multimodal
  
  
% Unsupervised learning, or learning from unlabelled data, enables using large scale datasets with no annotation effort. One important application of unsupervised learning is representation learning, where the goal is to obtain compressed representations of the data that contain all the relevant semantic aspects. The fundamental problem in representation learning is to decide what information is discarded or preserved to construct useful representations.

\begin{figure}[t]
\caption{The \method diagram. The backbone $f$ yields a 2d representation for each transformed image $f(\tau_g(\vx))$. Then the group marginal (green) is obtained by summing the rows and softmaxing (sm), and is compared to the prescribed target (red). Secondly, the content is obtained by summing the columns, and contrasted with the other view. The final representation for downstream tasks is the 2d one, which has been optimized through its marginals.}
\centering
\label{fig:schema}
\vskip 0.1in
\includegraphics[width=\columnwidth]{media/diagram_1group_vm3.pdf}
\vskip -0.1in
\end{figure} 

\todo{Chen: Improve Fig 1: 1) Notations are wrong: cols should be rows, and rows should be cols. 2) Better to mention within the figure which part is content and which is group? 3) For completeness, should we draw projector h and show h(c1) and h(c2)?}

The field of representation learning has evolved at a fast pace in recent years, partially due to the popularity of Multiview Self-Supervised Learning (MSSL). The main idea of MSSL is to learn transformation-invariant representations by comparing differently transformed data views. The underlying hypothesis is that the transformations applied introduce task-irrelevant information, thus multiple views of the same data should yield similar representations that only contain task-relevant information. Such an idea is often put into practice with variants of the InfoNCE loss \cite{cpc}, popularly named as contrastive MSSL approaches \cite{simclr, moco, swav}, where views of the same image are contrasted with views of other images. Alternatively, other works explore MSSL from a non-contrastive perspective, by only comparing pairs of the same image \cite{byol, btwins}. 
%In these works, additional regularization is required, such as encoding one of the views with a shifted and frozen version of the main encoder. 
\todo{Do we need to mention contrastive and non-contrastive?}
 
The end goal of MSSL is to learn generic representations useful for \textit{any} downstream task. Thus, the input transformations should be diverse enough to generate informative views, and also carefully selected so that task-relevant information is preserved at the representation level. However, both requirements are impossible to satisfy in practice, and one can always find a downstream task for which the chosen transformations are ineffective. For example, MSSL representations learnt to be color invariant will fail for the task of predicting fruit ripeness (color information is required). Moreover, multiple transformations are typically applied at once (transformation stacks), which increases the number of ill-posed downstream tasks. Beyond classification or regression, MSSL may remove too much detail for other tasks such as generation or segmentation \cite{hybgencon}. 
%Summarizing, MSSL representations are tailored to work for tasks that do not require information related to the input transformations used.
%Many works have explored the most suitable transformations stacks for both supervised learning and MSSL \cite{fastaugment, autoaugment, randaugment, populationaugment}. However, the outcome of these works is still unclear \cite{arno_aug}.

One strategy to maintain information in the representations is by structuring them. This approach stems from observations in neuroscience related to the redundancy-reduction principle \cite{redundancyrevisited,perrone201531}. According to this principle, systems will learn organized representations, so that the capacity is not wasted in redundant features. \todo{better rephrase}
The redundancy-reduction principle has already inspired successful works in the unsupervised learning domain. For example, the TVAE \cite{tvae} proposes a VAE alternative that self-organizes the representations in an unsupervised way. Such structure preserves more information and proves helpful for generative tasks. 

Another strategy to preserve information in representations is via equivariance. Equivariant models  \cite{gcnn, sesn, arblie, qtae, offseteq} exploit symmetries in the data that can be expressed as algebraic groups. For example, \cite{sesn} proposes to use a basis of transformed filters to learn equivariant features.
% Note that one can still achieve the desired invariance by training a final layer on top of the equivariant representations. 
Equivariance has led to improved robustness both for supervised learning and MSSL \cite{essl, augself, hssl}. For MSSL, the recent works ESSL \cite{essl} and AugSelf \cite{augself} both make representations sensitive to a transformation by regressing to the transformation parameter. However, these methods do not yield structured representations. While ESSL representations can be theoretically equivariant, there is no explicit form of the transformation at representation level. On the other hand, NPTN \cite{nptn} learns structured representations with a basis of unsupervisedly learned filters. Unfortunately, NPTN loses the equivariance property. \todo{Chen: the introduction is a bit too long. I have trimmed it following the current flow. May come back for a rewrite if given enough time.}

% One strategy to enhance task-relevant information in MSSL is to encourage discarding task-irrelevant information. For example, with an explicit loss \cite{SSL_MV} or relaxing the invariance constraint by allowing a residual when comparing representations \cite{residualssl}. However, the underlying problem of knowing which invariances to learn is still present. Instead of discarding information, equivariant models preserve both task-relevant and task-irrelevant information in the representations \cite{gcnn, arblie, qtae, offseteq, tvae}. These models exploit symmetries in the data that can be expressed as algebraic groups. Note that one can still achieve the desired invariance by training a final layer on top of the equivariant representations. Furthermore, equivariant models show improved robustness both for supervised learning (SL) \cite{gcnn, sesn} and MSSL \cite{essl, hssl}. 
% However, equivariant models have some drawbacks: (1) they are designed for finite groups, where the number of group elements is usually small (\eg $90^{\circ}$ rotations), (2) suppose an increase in compute time and memory and (3) to the best of our knowledge do not perform well for non-exact algebraic groups (\eg color-related transformations).% or compositions of groups.

%and have been, etc. Not clear if features specific to each transformation are encouraged to learn, or just the augmentation information is transferred to the representation. \textit{Extreme case example, one float regresses the augmentation parameter and the remaining of the features stay the same. }
%Equivariant neural networks \cite{GCNN, SESN, etc} learn structured representations by using transformed versions of CNN filters, yielding representations specific to each group element. Equivariant models have some drawbacks: (1) they are designed for finite groups, where the number of group elements is usually small (\eg $90^{\circ}$ rotations), (2) suppose an increase in compute time and memory and (3) to the best of our knowledge do not perform well for color-related transformations or compositions of more than 2 groups.


In this work, we devise a method to learn both structured and equivariant representations with MSSL, which we call \method representations. Instead of using 1-dimensional representations, we learn 2-dimensional ones that allow for much richer structure. One axis of our representations is related to \textit{content} and the other one to \textit{group element}. The group element refers to how an input transformation is parameterized (\eg rotations of $90^\circ$) while the content includes all the information that is invariant to the group actions.
% We model the joint distribution over \textit{content} ($\sC$) and \textit{group} ($\sG$) element using MSSL.
% The group element defines the input transformation applied, while the content includes all the information in the image that is invariant to the group actions. 
Our formulation allows a natural marginalization of content and group, which can be maximized separately as shown in Figure \ref{fig:schema}. We maximize the content marginal by maximizing agreement between two views of the same image as in SimCLR \cite{simclr}. The group marginal is matched to a known target distribution by means of Jensen-Shannon Divergence. The resulting \method representations are structured in terms of group elements, and we show both theoretically and empirically that they are also equivariant under specific training conditions. Furthermore, \method (i) can naturally handle finite and infinite groups, (ii) has minimal impact on  the compute time and (iii) can be extended to learn structure for an arbitrary number of groups.

% Additionally, we show that \method representations are explicitly equivariant and can be transformed analytically in feature space, as opposed to \cite{essl, augself}.

Our experiments show that \method consistently improves the top-1 performance of SimCLR. We also compare favorably with ESSL (equivariant representations) and a \method variant that resembles NPTN (structured representations), showing the importance of both structure and equivariance. Furthermore, \method representations drastically improve generative performance (up to $3\times$ better reconstruction error than SimCLR) and achieve better downstream performance on a large set of classification tasks. Finally, \method allows direct recovery of the transformation parameter of an arbitrary image, without requiring any specialized regression head as in \cite{essl, augself}. \todo{Rewrite summary of results.}

% Representations learnt with \method improve top-1 test performance compared to a SimCLR \cite{simclr} baseline. We also improve performance for all group-specific augmentations tested, and we compare favorably with NPTN \cite{nptn} and ESSL \cite{essl}.
% We additionally show that \method representations drastically improve generative performance (up to $3\times$ better reconstruction error than SimCLR representations) and better downstream performance to a large set of classification tasks. Finally, \method allows direct recovery of the input transformation parameter of an arbitrary image, without requiring any specialized regression head or classifier (as in \cite{essl, augself}), which improves interpretability.
% One key aspect of equivariant networks is that they learn a representation \textit{per finite group element}. Therefore, an image is represented by the aggregation of the representations for all group elements. Inspired by this over-complete aspect of equivariant representations we propose \method, a new method to learn an over-complete representation that addresses the drawbacks mentioned for equivariant networks: (1) naturally handles continuous groups, (2) does not increase the compute time and (3) we show theoretically and empirically how structure is learnt jointly for an arbitrary number of groups. \method's core idea is to treat the latent representation of our SSL backbone as a joint probability distribution over \textit{content} ($\sC$) and \textit{group} ($\sG$). The group defines the input transformation applied, while the content includes all the  information of the image that is invariant to the group actions. Our formulation allows an easy marginalization of content and group, which can be maximized separately. We maximize the content marginal distributions between two views using a contrastive loss as in \cite{simclr}, and to match the marginal group distribution to a Gaussian target. The resulting joint representation learnt is structured both in terms of content (features describing the images) and group elements. 
In summary, our main contributions are \todo{Update}:
\begin{itemize}
    \item A method to incorporate structure in MSSL representations for both finite and infinite groups with negligible computational overhead. Our approach also performs well for parameterized transformations that do not satisfy all algebraic group axioms, making it widely applicable to all transformations used in MSSL.
    \item We show theoretically and empirically that \method representations are also equivariant when our group marginal loss is satisfied. \todo{talk about bound?}
    \item We show that \method outperforms the representative methods SimCLR, NPTN and ESSL for diverse groups on the CIFAR10/100 and TinyImageNet datasets. Importantly, \method performs successfully with color transformations, while ESSL does not.
    \item We shed some light on why certain symmetries are harder to learn from typical computer vision datasets.
    
    % \item \method, a method to learn the structured representations for arbitrary (finite and infinite) groups with no computational overhead. Our approach also performs well for parameterized transformations that do not satisfy all algebraic group axioms, making it widely applicable to all transformations used in MSSL.
    % \item Extensive experiments on MNIST, CIFAR10, CIFAR100 and TinyImageNet; showing the benefits of using \method representations for classification and generation in the MSSL setting.
    % \item A theoretical formulation and empirical validation of equivariance learnt using \method.
    % \item We further show how equivariance can be exploited for conditioned image generation.
    % \item Our method also strongly improves the efficacy of self-supervised features for generative purposes. We show that the reconstruction error is drastically reduced with respect to SimCLR feature. Moreover, we show reconstruction can be easily controlled thanks to the equivariance properties of our features.
    % \item Allows 0-shot regression of the augmentation parameters applied on a test image! 
    % \item An analysis on the coupling of different augmentations, hinting which augmentations are actually useful.
\end{itemize}

% Ideas:
% \begin{itemize}
%     \item Can we beat ESSL for gray-scale, blur, flip, etc.? Running in \texttt{moedec3k-A0fli}.
%     \item Implement ESSL as second baseline! Show MSE and parameter regression performance.
%     \item Check if we can regress parameters for joint groups.
% \end{itemize}



==> sections/results.tex <==

\begin{figure*}[htb]

\caption{Empirical validation of equivariance in \method. We measure the L2 distance between the representations of a transformed image $f(\tau_g(\vx))$ and the transformed representations of that image $T_g(f(\vx))$, varying $g \in [0,1]$ along both axes. The plots show the average L2 distance for 1000 CIFAR-10 test images. Note the strong similarity for the same group element (diagonal), and the cyclic nature of rotations or flips when using a $\VM$ target (\textbf{top row}), as opposed to the Gaussian target (\textbf{bottom row}). More results in \Cref{app:empiricalequivariance}.}
\label{fig:empiricaleq}

\centering
\begin{subfigure}{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{media/equivariance/rotation180_shujr5wn2a_equi_dist_matrix_meanshift_vm_3.0.png}
    % \caption{Firts subfigure.}
\end{subfigure}%
\hfill
\begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/rotation4f_2crx6y3u6s_equi_dist_matrix_meanshift_vm_3.0.png}
    % % \caption{Third subfigure.}
\end{subfigure}%
\hfill
\begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/hflip_jfvvcwmmkx_equi_dist_matrix_meanshift_vm_3.0.png}
    % \caption{Third subfigure.}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/vflip_3ksvgzny84_equi_dist_matrix_meanshift_vm_3.0.png}
    % \caption{Third subfigure.}
\end{subfigure}


\vspace{-4mm}
% \vfill

\centering
\begin{subfigure}{0.195\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/brightness_q4h8fu9iak_equi_dist_matrix_meanshift_ga_0.2.png}
    % \caption{Firts subfigure.}
\end{subfigure}
\hfill
\begin{subfigure}{0.195\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/contrast_g5w4b3u7x4_equi_dist_matrix_meanshift_ga_0.2.png}
    % \caption{Second subfigure.}
\end{subfigure}
\hfill
\begin{subfigure}{0.195\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/saturation_vkigwy2fqh_equi_dist_matrix_meanshift_ga_0.2.png}
    % \caption{Third subfigure.}
\end{subfigure}
\hfill
\begin{subfigure}{0.195\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/hue_jfidfyw9rf_equi_dist_matrix_meanshift_ga_0.2.png}
    % \caption{Third subfigure.}
\end{subfigure}
\hfill
\begin{subfigure}{0.195\textwidth}
    \includegraphics[width=\textwidth]{media/equivariance/grayscale_d53q8wx8tv_equi_dist_matrix_meanshift_ga_0.2.png}
    % \caption{Third subfigure.}
\end{subfigure}
\vspace{-4mm}

\end{figure*}

\section{Experimental Results}

\subsection{Empirical Proof of Equivariance}
\label{sec:empiricalequivariance}

We start with an empirical validation of equivariance by measuring how \cref{eq:equivariance} holds for real data. For that, we use the transformation $T_g$ from \cref{eq:t_g} and compute representations $f(\tau_{g_1}(\vx))$ and $T_{g_2}(f(\vx)) \;\forall g_1,g_2\in\sG$. An equivariant map should result in a minimal L2 distance $\ell_{g_1,g_2} = \| f(\tau_{g_1}(\vx)) - T_{g_2}(f(\vx)) \|_2^2$ when $g_1=g_2$ \todo{Careful: our notion of equivariance is linked to the group marginal: we can't hope (in general) that the equivariance condition holds at feature space $\vz$; we can, however, hope that it matches at its column-reduction $\mu$. That is to say, I think it would be more consistent if you compared $\| \sum_i f(\tau_{g_1}(\vx))_{ij} - T_{g_2}(f(\vx))_{ij} \|_2^2 = \|\mu(\tau_{g_1}(\vx)) - \mu(T_{g_2}(f(\vx)))\|_2^2$. Actually, I'm quite impressed that the feature-space error is small at all! This hints at the fact that there's some implicit regularisation going on under the hood, which forces the whole feature space to follow equivariance, too! Amazing!}. To verify that, we plot the pairwise $\ell_{g_1,g_2}$ for all elements $g_1,g_2$ and different transformations. More precisely, we sweep 100 values of $g_1, g_2$ in $[0, 1]$ for 1000 randomly selected CIFAR-10 \cite{krizhevsky2009learning} test images and we show the average pairwise L2 distance in \Cref{fig:empiricaleq}.

For infinite groups (\ie color transformations and rotation ($360$)), there is a strong similarity along the diagonal, validating \cref{eq:equivariance}. For finite groups (rotation 4-fold, flips and grayscale) we also see a strong similarity at the observed group elements. For example, rotation 4-fold shows 4 minima at the observed (normalized) angles. These plots also help to understand how the model generalizes to unseen group elements. 
Interestingly, equivariance for horizontal flip is mildly learnt due to its ambiguity in the dataset (see \Cref{sec:ambiguity} for extended discussion). 
Indeed, flipped images appear naturally in CIFAR-10 (\eg{} cars looking to the right or left), and thus there is more ambiguity about the meaning of image flipping. On the other hand, vertical flips are nicely learnt, since they do not naturally appear in data. Another interesting observation is that grayscale yields a constant representation as we reduce the saturation (horizontal axis) and then shows a sudden jump close to 1 (grayscale image). The model has learnt that any image with \textit{some} color is \textit{not} grayscale, unless it is purely grayscale. Note that grayscale does not form an algebraic group, yet \method is able to learn its structure.
% Also note how the $VM$ target (top row) helps learning the cyclic nature of rotations and flips, as opposed to the Gaussian target (see \Cref{app:empiricalequivariance}).




\begin{figure}[tb]
\caption{Equivariance in \method. We encode a test image (leftmost images), transform its representation using $T_g$ (\cref{eq:t_g}) with several $g$, and then decode the transformed representations. See how transforming the representations exposes the input transformation learnt by the model, empirically proving equivariance.}
\centering
\label{fig:decoded_mnist_cifar}
\vskip 1mm
\begin{subfigure}[b]{1.0\columnwidth}
    \includegraphics[height=22.5mm]{media/decoded/decoded_v4gi5yxnfw_rot180_mnist_vm.png}\hfill
    \includegraphics[height=22.5mm]{media/decoded/decoded_vabqg57skq_fli_mnist_vm_gamma.png}
    \caption{MNIST with \textit{Rot. (360)} (left) and \textit{horizontal flip} (right).}
\end{subfigure}
\vskip -1.7mm
\begin{subfigure}[b]{1.0\columnwidth}
    \includegraphics[width=\columnwidth]{media/decoded/decoded_5.jpg}
    \caption{CIFAR-10 for \textit{Rot. (360)} and \textit{color} transformations.}
\end{subfigure}
\vskip -0.2in
\end{figure}

\subsection{\method Representations for Group Conditional Generation}
\label{sec:generation}

We study the benefit of equivariance in \method representations to conditioning generation on specific group elements. 
To that end, we train a detached (stop-grad) decoder on frozen pre-trained \method representations. 
% To that end, we train a detached (stop-grad) decoder on top of our \method representations provided by a frozen pre-trained \method backbone. 
In this work we do not aim to obtain state-of-the-art generation quality, but rather use a decoder for visual validation of our hypotheses. Note that group conditional generation is not feasible with MSSL methods like SimCLR or ESSL since there is no explicit transformation at representation level.

Here we exploit the equivariant property of \method representations for controlled generation. We first obtain the representation of a test image $\vz = f(\vx)$ (leftmost images in \Cref{fig:decoded_mnist_cifar}), then we create multiple transformed representations $\{T_g(\vz)\}$ using \cref{eq:t_g}, by sweeping $g$ between $0$ and $1$, and finally we decode all $\{T_g(\vz)\}$. In \Cref{fig:decoded_mnist_cifar} we show the decoded images for different datasets and groups. Note how we can recover the input transformation by only transforming the representations, yet an additional visual proof of equivariance in \method. In \Cref{app:rec_error} we also show that reconstruction error obtained with \method is up to 66\% smaller than with SimCLR (rotation (4-fold)) and up to 70\% smaller than with ESSL (grayscale).



\subsection{\method Representations for Classification}
\label{sec:rep-cls}
\subsubsection{RRC+1 Experiments}
\label{RRC+1}


\begin{figure*}[tb]
\caption{Test top-1 performance of a linear tracking head on CIFAR-10. It can be observed that \method improves over SimCLR and ESSL for all transformations. Notably for continuous color transformations, ESSL significantly degrades performance unlike \method.}
\centering
\label{fig:cifar10_top1}
\includesvg[width=0.9\textwidth]{media/top1/CIFAR-10.svg}
\vskip -0.3in
\end{figure*}

In this section we analyze how \method representations perform for discriminative tasks. Following ESSL where a single transformation is applied on top of RandomResizedCrop (RRC), we carry out the set of {RRC+1} experiments. We compare our method with SimCLR and ESSL. 
Recall that ESSL representations are implicitly equivariant but do not guarantee interpretable structure with respect to the transformation.
% Recall that ESSL preserves the transformation information by training an additional regression head ($\lambda=0.4$ by default). Therefore, ESSL representations are only implicitly equivariant and do not guarantee interpretable structure with respect to the transformation.
We also compare with a variant of our method with $\lambda=0$ (\stovez). In \stovez we still reshape the features to 2d and sum over the columns to obtain the content representation (that is contrasted), which is a fundamental difference with SimCLR. \stovez learns unsupervised invariances very similarly to what NPTN \cite{nptn} does, but does not guarantee equivariance.
For RRC+1, \method uses $\lambda=10$, except for \textit{rotations} and \textit{vertical flip} for which we use $\lambda=1000$ according to the empirical study in \Cref{sec:ablation}. We set $\sigma=0.2$ and $\dg=8$. The full training procedure is provided in \Cref{sec:train_procedure}.

In \Cref{fig:cifar10_top1} we show the accuracy of a linear tracking head for the RRC+1 experiment on CIFAR-10. The horizontal dashed line shows the baseline performance of SimCLR with only RRC. For \method, the tracking head receives our 2d representation flattened, being of the \textit{same dimensionality} as in compared methods. Our method outperforms SimCLR for all transformations, and even improves over SimCLR with RRC only by learning structure with respect to scale. Note that, by construction, ESSL cannot improve over the RRC-only baseline. 

A prominent result is the performance of \method with color transformations. For the discrete transformation \textit{grayscale}, ESSL degrades performance by 12.8\% with respect to SimCLR with grayscale, while \method improves by 1.75\%. %The ESSL result for \textit{grayscale} is inline with the results reported in \cite{essl}.
For continuous color transformations, \method improves over SimCLR between 3-5\%, while ESSL degrades the performance by up to 4.3\% (brightness). This shows that the implicit equivariance learnt by ESSL is not sufficient.

We also observe in \Cref{fig:cifar10_top1} that learning structure for horizontal flips with ESSL or \method~($\mathcal{N}$) does not improve over SimCLR, given the ambiguity of the transformation (see \Cref{sec:ambiguity}). However, \method~($\VM$) improves over SimCLR by 2.8\%, similar to \stovez, hinting that structure is helpful if it reflects the nature (cyclic) of the transformation. Otherwise, it is beneficial to learn unsupervised structure (\stovez). We also see that structure (and equivariance) is strongly helpful for vertical flips.
%Interestingly, and coherent with the ESSL paper results, structure (or equivariance) is beneficial with vertical flips.
For the more complex cyclic transformations, \stovez underperforms by a large margin, since such complex structure is harder to learn unsupervisedly. This result shows that accounting for the topological structure of the transformation (as studied  by \citet{homeomorphic}) is of great importance, and opens the door to further research in this direction. 
Surprisingly, \stovez outperforms SimCLR. We speculate that the unsupervised structure learnt by \stovez might induce a more discriminative organization of the embedding space.


% The structure learnt by \method is beneficial for classification and performs consistently for all groups tested. ESSL also outperforms SimCLR for some transformations (rotations and vertical flip), but does not perform consistently for color transformations.
\Cref{tab:RRCp1} benchmarks the more complex tasks CIFAR-100 \cite{krizhevsky2009learning} and TinyImageNet \cite{tin}. \method achieves the highest accuracy compared to all algorithms tested, including \stovez, and across all groups. \method also improves under color transformations with respect to SimCLR with the same transformations, while ESSL shows a degradation. Indeed, the datasets used in \Cref{tab:RRCp1} present higher data scarcity per class than CIFAR-10. In such setting, the structure learnt by \method shines over unstructured methods like ESSL.

\subsubsection{Full Augmentation Stack Experiments}
\label{sec:fullstack}

In this section we use the full augmentation stack as in SimCLR (see details in \Cref{app:fullstack-augs}). We learn structure for one group at a time, while applying the full stack on input images. Note that in the full stack setting, we use a fixed $\lambda=10$ for \method\footnote{We did not perform an extensive hyper-parameter tuning, the focus of this work being an exploration of structured representations in MSSL.}. We observed in this case that extremely large $\lambda$ can harm performance since multiple transformations add ambiguity to the group being learnt. 

\Cref{tab:fullstack} reports the test top-1 accuracy on CIFAR-10, CIFAR-100 and TinyImagenet. \method improves the performance over SimCLR (up to +1.1\%) and ESSL (up to 7.1\%) for all color transformations on CIFAR-100 and TinyImageNet (up to 2.2\% and 7.05\% respectively). The performance is on par with SimCLR and \stovez on CIFAR-10. Conversely, color transformations adversely affect ESSL, and the performance is degraded by up to -6.61\% with respect to SimCLR (\textit{grayscale} on TinyImageNet).

Interestingly, neither \method nor ESSL outperform SimCLR by becoming equivariant to horizontal flips, as discussed in \Cref{sec:ambiguity}. Nevertheless, \method still outperforms ESSL for horizontal flips by 0.37\%, 5.1\% and 2.94\% on CIFAR-10, CIFAR-100 and TinyImageNet respectively. Similarly, as the dataset complexity increases, \method performs better than ESSL for vertical flips.
Another interesting result is the effectiveness of ESSL with rotations, where \method remains subpar but better than the SimCLR baseline. 

To grasp the overall performance, we show the average across groups in the \textit{Avg.} column\footnote{For \method we compute the average using the recommended target distributions in \Cref{tab:groups}.}. \method achieves the best average for TinyImageNet, and the relative gap with respect to SimCLR and ESSL increases with the dataset complexity. It is surprising how well \stovez performs in the full stack setting, achieving similar performance as \method. However, having structure regularization is still beneficial, especially when dealing with more complex data. 
% Overall, \Cref{tab:fullstack} shows how \method's structure and equivariance is extremely helpful when observations about the group elements are scarcer (\eg less data or increased data diversity).

\addtolength{\tabcolsep}{-1pt}    
\begin{table*}[tb]
    \caption{RRC+1 results: Top-1 accuracy of a linear tracking head on CIFAR-100 and TinyImageNet. \method improves over SimCLR for all groups, while ESSL worsens performance for color transformations. Note the benefits of accounting for the cyclic nature of rotations and flips using a $\VM$ target. We report the $\text{mean}_{\text{std}}$ over 3 runs.} 
    \label{tab:RRCp1}
    \scriptsize
    % \centering
    % \ra{1.0}
    % \hskip 0.015in
    \vskip 0.1in
    \begin{tabularx}{\textwidth}{@{}Xlcccccccccc@{\hspace{2mm}}|@{\hspace{2mm}}c}
    % \begin{tabularx}{\textwidth}{XXXXXXXXXXXX}
    \toprule
    Dataset & Method &  RRC & Rot. (360) &   Rot. (4-fold) &         H. Flip &         V. Flip &               Grayscale &              Brightness &                Contrast &             Saturation &                     Hue & Avg. \\
    \midrule
%     \multirow{4}{*}{CIFAR-10} & SimCLR                &           69.87 &           55.51 &           61.12 &           70.78 &           64.89 &                   79.59 &                   75.44 &                   74.99 &                  72.77 &                   73.52 \\
% & ESSL                  &               - &           70.59 &           76.52 &           70.25 &            74.0 &  \textcolor{black}{67.33} &  \textcolor{black}{52.58} &  \textcolor{black}{43.11} &  \textcolor{black}{40.7} &  \textcolor{black}{49.84} \\
% & STOVE ($\mathcal{N}$) &  \textbf{74.53} &           70.77 &           77.42 &           71.28 &           77.69 &          \textbf{81.34} &          \textbf{77.65} &          \textbf{77.78} &         \textbf{76.24} &           \textbf{77.5} \\
% & STOVE (VM)            &               - &  \textbf{73.46} &  \textbf{77.84} &  \textbf{73.54} &  \textbf{77.85} &                       - &                       - &                       - &                      - &                       - \\


%     \midrule
    \multirow{4}{*}{CIFAR-100}  & SimCLR               &           38.89\textsubscript{0.26} &           32.17\textsubscript{0.14} &           35.52\textsubscript{0.33} &           39.85\textsubscript{0.13} &           36.68\textsubscript{0.27} &           47.41\textsubscript{0.40} &           45.00\textsubscript{0.26} &           44.51\textsubscript{0.04} &           42.27\textsubscript{0.70} &           43.61\textsubscript{0.19} &           40.59\textsubscript{0.22} \\
& ESSL                 &                        - &           38.03\textsubscript{0.36} &           44.36\textsubscript{0.72} &           38.78\textsubscript{0.54} &           42.17\textsubscript{0.87} &           34.20\textsubscript{0.60} &           38.33\textsubscript{0.25} &           38.66\textsubscript{0.02} &           38.92\textsubscript{0.08} &           37.64\textsubscript{0.39} &           39.01\textsubscript{0.35} \\
& \stovez   &           42.63\textsubscript{0.11} &           34.77\textsubscript{0.72} &           38.28\textsubscript{0.19} &  \textbf{43.54}\textsubscript{0.67} &           40.10\textsubscript{0.82} &           48.87\textsubscript{0.18} &           48.12\textsubscript{0.19} &           47.74\textsubscript{0.57} &           45.39\textsubscript{0.34} &           46.32\textsubscript{0.61} &           43.57\textsubscript{0.36} \\
& \method ($\mathcal{N}$) &  \textbf{45.25}\textsubscript{0.10} &           39.53\textsubscript{0.71} &           45.54\textsubscript{0.45} &           43.24\textsubscript{0.13} &  \textbf{45.98}\textsubscript{0.56} &  \textbf{50.91}\textsubscript{0.49} &  \textbf{50.18}\textsubscript{0.45} &  \textbf{49.77}\textsubscript{0.46} &  \textbf{48.75}\textsubscript{0.22} &  \textbf{48.54}\textsubscript{0.78} & \multirow{2}{*}{{\textbf{46.97}\textsubscript{0.35}}} \\
& \method ($\VM$)            &                        - &  \textbf{42.17}\textsubscript{0.42} &  \textbf{47.25}\textsubscript{0.26} &           41.82\textsubscript{0.46} &           45.38\textsubscript{0.73} &                        - &                        - &                        - &                        - &                        - &            \\

    \midrule
    \multirow{4}{*}{TinyImageNet}   & SimCLR               &           26.91\textsubscript{0.13} &           21.34\textsubscript{0.08} &           24.40\textsubscript{0.24} &           27.90\textsubscript{0.37} &           26.74\textsubscript{0.30} &           31.35\textsubscript{1.29} &           29.95\textsubscript{0.14} &           29.68\textsubscript{0.18} &           28.60\textsubscript{0.29} &           28.20\textsubscript{0.40} &           27.50\textsubscript{0.28} \\
& ESSL                 &                        - &           25.35\textsubscript{0.10} &           30.41\textsubscript{0.25} &           27.13\textsubscript{0.14} &           29.11\textsubscript{0.27} &           23.51\textsubscript{0.18} &           26.45\textsubscript{0.07} &           26.32\textsubscript{0.61} &           26.75\textsubscript{0.72} &           26.00\textsubscript{0.11} &           26.78\textsubscript{0.22} \\
& \stovez   &           29.57\textsubscript{0.47} &           24.22\textsubscript{0.30} &           26.96\textsubscript{0.37} &  \textbf{30.78}\textsubscript{0.23} &           28.98\textsubscript{0.42} &           31.55\textsubscript{0.14} &           32.54\textsubscript{0.18} &           32.23\textsubscript{0.17} &           31.43\textsubscript{0.24} &           30.45\textsubscript{0.60} &           29.87\textsubscript{0.25} \\
& \method ($\mathcal{N}$) &  \textbf{31.26}\textsubscript{0.21} &           26.00\textsubscript{0.28} &           30.97\textsubscript{0.43} &           30.15\textsubscript{0.26} &  \textbf{32.04}\textsubscript{0.29} &  \textbf{34.92}\textsubscript{0.24} &  \textbf{33.96}\textsubscript{0.16} &  \textbf{34.20}\textsubscript{0.34} &  \textbf{33.42}\textsubscript{0.35} &  \textbf{32.64}\textsubscript{0.03} &  \multirow{2}{*}{{\textbf{32.18}\textsubscript{0.21}}} \\
& \method ($\VM$)            &                        - &  \textbf{27.78}\textsubscript{0.24} &  \textbf{31.55}\textsubscript{0.28} &           30.34\textsubscript{0.59} &           31.71\textsubscript{0.53} &                        - &                        - &                        - &                        - &                        - &            \\


    \bottomrule
\end{tabularx}
\end{table*}
\addtolength{\tabcolsep}{1pt}   




\addtolength{\tabcolsep}{-1pt}    
\begin{table*}[tb]
    \caption{Results for the full augmentation stack experiment, test accuracy of a linear tracking head. Columns \textit{Rot. (360)}, \textit{Rot. (4-fold)} and \textit{V. Flip} require an additional transformation. We report the $\text{mean}_{\text{std}}$ over 3 runs.}
    \label{tab:fullstack}
    \scriptsize
    % \centering
    % \ra{1.0}
    % \hskip 0.015in
    \vskip 0.1in
    \begin{tabularx}{\textwidth}{@{}Xlcccccccccc@{\hspace{2mm}}|@{\hspace{2mm}}c}
    \toprule
    Dataset & Method &  RRC & Rot. (360) &   Rot. (4-fold) &         H. Flip &         V. Flip &               Grayscale &              Brightness &                Contrast &             Saturation &                     Hue & Avg. \\
    \midrule
    \multirow{4}{*}{CIFAR-10} & SimCLR               &  87.42\textsubscript{0.01} &           79.90\textsubscript{0.50} &           81.50\textsubscript{0.44} &  87.48\textsubscript{0.06} &           82.78\textsubscript{0.23} &  87.41\textsubscript{0.03} &  \textbf{87.51}\textsubscript{0.11} &  \textbf{87.57}\textsubscript{0.19} &  87.49\textsubscript{0.08} &           87.67\textsubscript{0.34} &           85.67\textsubscript{0.14} \\
& ESSL                 &               - &  \textbf{86.55}\textsubscript{0.13} &  \textbf{89.33}\textsubscript{0.32} &  84.78\textsubscript{0.40} &  \textbf{86.66}\textsubscript{0.21} &  83.59\textsubscript{0.43} &  85.78\textsubscript{0.25} &  86.31\textsubscript{0.16} &  87.12\textsubscript{0.30} &           86.39\textsubscript{0.44} &  \textbf{86.28}\textsubscript{0.24} \\
& \stovez   &  \textbf{87.50}\textsubscript{0.20} &           79.05\textsubscript{0.37} &           81.32\textsubscript{0.18} &  \textbf{87.73}\textsubscript{0.19} &           82.66\textsubscript{0.14} &  \textbf{87.69}\textsubscript{0.17} &           87.47\textsubscript{0.13} &           87.34\textsubscript{0.20} &  \textbf{87.54}\textsubscript{0.33} &           87.63\textsubscript{0.20} &           85.59\textsubscript{0.21} \\
& \method ($\mathcal{N}$) &  87.22\textsubscript{0.10} &           80.90\textsubscript{0.33} &           83.43\textsubscript{0.29} &  86.44\textsubscript{0.26} &           83.66\textsubscript{0.25} &  87.40\textsubscript{0.08} &  86.97\textsubscript{0.22} &  87.05\textsubscript{0.37} &  87.52\textsubscript{0.19} &  \textbf{87.97}\textsubscript{0.11} &           \multirow{2}{*}{85.88\textsubscript{0.18}} \\
& \method ($\VM$)            &               - &           81.70\textsubscript{0.30} &           83.49\textsubscript{0.16} &  85.64\textsubscript{0.08} &           83.84\textsubscript{0.22} &               - &               - &               - &               - &                        - &           \\


    \midrule
    \multirow{4}{*}{CIFAR-100}  & SimCLR               &           61.40\textsubscript{0.17} &           56.40\textsubscript{0.30} &           57.32\textsubscript{0.03} &  61.48\textsubscript{0.28} &           56.73\textsubscript{0.48} &           61.43\textsubscript{0.21} &           61.31\textsubscript{0.05} &  61.68\textsubscript{0.57} &           61.57\textsubscript{0.41} &           61.30\textsubscript{0.03} &           60.06\textsubscript{0.18} \\
& ESSL                 &                        - &  \textbf{58.32}\textsubscript{0.06} &  \textbf{63.28}\textsubscript{0.28} &  55.22\textsubscript{0.29} &           57.18\textsubscript{0.18} &           55.10\textsubscript{0.47} &           57.92\textsubscript{0.38} &  58.06\textsubscript{0.58} &           60.25\textsubscript{0.34} &           58.91\textsubscript{0.30} &           58.25\textsubscript{0.26} \\
& \stovez   &           62.13\textsubscript{0.13} &           55.49\textsubscript{0.22} &           57.79\textsubscript{0.40} &  \textbf{62.25}\textsubscript{0.34} &           56.88\textsubscript{0.18} &  \textbf{62.32}\textsubscript{0.26} &  \textbf{62.39}\textsubscript{0.27} &  \textbf{62.47}\textsubscript{0.16} &           62.54\textsubscript{0.20} &           62.29\textsubscript{0.29} &           \textbf{60.65}\textsubscript{0.24} \\
& \method ($\mathcal{N}$) &  \textbf{62.17}\textsubscript{0.28} &           55.82\textsubscript{0.40} &           58.02\textsubscript{0.47} &  60.84\textsubscript{0.03} &  \textbf{57.47}\textsubscript{0.22} &  {62.18}\textsubscript{0.51} &  {62.24}\textsubscript{0.31} &  61.90\textsubscript{0.72} &  \textbf{62.67}\textsubscript{0.19} &  \textbf{63.31}\textsubscript{0.21} &  \multirow{2}{*}{{60.52}\textsubscript{0.27}} \\
& \method ($\VM$)            &                        - &           55.66\textsubscript{0.39} &           58.01\textsubscript{0.31} &  59.62\textsubscript{0.11} &           57.40\textsubscript{0.15} &                        - &                        - &               - &                        - &                        - &            \\


    \midrule
    \multirow{4}{*}{TinyImageNet}   & SimCLR               &           42.16\textsubscript{0.16} &           37.35\textsubscript{0.19} &           39.23\textsubscript{0.15} &  {42.31}\textsubscript{0.06} &           38.50\textsubscript{0.09} &           42.11\textsubscript{0.23} &           42.32\textsubscript{0.08} &           42.34\textsubscript{0.10} &           42.27\textsubscript{0.01} &           42.46\textsubscript{0.27} &           41.11\textsubscript{0.09} \\
& ESSL                 &                        - &           37.53\textsubscript{0.21} &  \textbf{42.86}\textsubscript{0.29} &           36.25\textsubscript{0.13} &           37.18\textsubscript{0.77} &           35.50\textsubscript{0.30} &           37.94\textsubscript{0.13} &           38.66\textsubscript{0.50} &           40.55\textsubscript{0.74} &           40.49\textsubscript{0.05} &           38.55\textsubscript{0.28} \\
& \stovez  &           43.07\textsubscript{0.11} &           36.28\textsubscript{0.95} &           39.54\textsubscript{0.41} &  \textbf{42.43}\textsubscript{0.33} &           38.87\textsubscript{0.40} &  \textbf{42.79}\textsubscript{0.16} &           42.61\textsubscript{0.34} &           42.98\textsubscript{0.08} &           42.86\textsubscript{0.30} &           42.90\textsubscript{0.46} &           41.43\textsubscript{0.36} \\
& \method ($\mathcal{N}$) &  \textbf{43.56}\textsubscript{0.54} &  \textbf{38.27}\textsubscript{0.91} &           40.55\textsubscript{0.45} &           41.18\textsubscript{0.94} &           39.17\textsubscript{0.51} &           42.55\textsubscript{1.27} &  \textbf{43.41}\textsubscript{0.01} &  \textbf{43.71}\textsubscript{0.07} &  \textbf{44.13}\textsubscript{0.57} &  \textbf{44.61}\textsubscript{0.10} &  \multirow{2}{*}{\textbf{41.91}\textsubscript{0.41}} \\
& \method ($\VM$)            &                        - &           38.06\textsubscript{0.06} &           40.03\textsubscript{0.28} &           40.43\textsubscript{0.21} &  \textbf{39.36}\textsubscript{0.50} &                        - &                        - &                        - &                        - &                        - &            \\

    \bottomrule
\end{tabularx}
\end{table*}
\addtolength{\tabcolsep}{1pt}   


\subsection{Transfer to Other Datasets}
\label{sec:transfer}

\todo{New ESSL results in q453xm539a.}One key goal of representation learning is to obtain representations that transfer to other tasks. We evaluate how \method, SimCLR and ESSL representations (trained on TinyImageNet) transfer to several classification  tasks in the RRC+1 setting (full tables and ESSL results in \Cref{app:transfer}).

\method's structure to rotations yields a gain of +21\% with respect to SimCLR when transferring to Caltech101 \cite{caltech101}, and between +5.97\% and +16.97\% when transferring to other datasets like CIFAR-10, CIFAR-100, DTD \cite{dtd} or Oxford Pets \cite{pets}. Structure to color transformations also proves beneficial, with a +6.36\% gain on Flowers \cite{flowers} (grayscale), Food101 \cite{food101} (hue) and +7.13\% on CIFAR-100 (hue). Horizontal flip is the transformation that sees less gain due to its ambiguity, as discussed in \Cref{sec:ambiguity}.

% It is interesting to see that \method achieves slightly worse performance for rotations or flips on the Flowers dataset. Indeed, this dataset contains many \textit{circular} flowers, which are rotation (or flip) invariant. In such situation, learning structure for rotations (or flips) should not give any gain. Actually, in \method we are trading off content for structure, so if the structure learnt is not useful, we are actually diminishing the expressivity of the final representations.

% \begin{figure}[tb]
% \caption{Difference in accuracies between \method and SimCLR, when transferring representations learnt on TinyImageNet to different datasets in the RRC+1 setting.}
% \centering
% \label{fig:transfer}
% \includesvg[width=\columnwidth]{media/transfer/transfer_tin_STOVE - SimCLR.svg}
% \vskip -0.2in
% \end{figure}

% One key goal of representation learning is to obtain representations that transfer to other tasks. We evaluate how \method, SimCLR and ESSL representations (trained on TinyImageNet) transfer to several classification downstream tasks in the RRC+1 setting. 
% More precisely, we train a logistic regression classifier on the representations of the training split of each dataset. No augmentations are applied during the classifier training. At test time, we evaluate the classifier on the test set of each dataset.
% %and the logistic regression is trained at once (using the full dataset).

% In \Cref{fig:transfer} we report the difference in accuracies between \method and SimCLR.
% \method's structure to rotations yields a gain of +21\% when transferring to Caltech101, and very important gains when transferring to other datasets like CIFAR-10, CIFAR-100, DTD or Pets. Structure to color transformations also proves beneficial, with a +6.36\% gain on Flowers (grayscale) and 7.13\% on CIFAR-100 (hue). Horizontal flip is the transformation that sees less gain.

% It is interesting to see that \method achieves slightly worse performance for rotations or flips on the Flowers dataset. Indeed, this dataset contains many \textit{circular} flowers, which are rotation (or flip) invariant. In such situation, learning structure for rotations (or flips) should not give any gain. Actually, in \method we are trading off content for structure, so if the structure learnt is not useful, we are actually diminishing the expressivity of the final representations. We also provide additional results in \Cref{app:transfer}.






==> sections/sota.tex <==
\section{Related Work}

\textbf{Information preservation} The key goal in representation learning is to preserve as much information as possible about the input, as stated by the InfoMax principle \cite{InfoMax}. The recent success of MSSL can be similarly explained from the perspective of mutual information maximization \cite{admim}, \ie maximizing mutual information between the representations of multiple data views. However, the popular MSSL methods based on contrastive learning may discard important task-relevant features (\ie feature suppression) when they throw out nuisance features at the same time. Hence, contrastive learning is often combined with some reconstruction loss \cite{pcl_feature_suppression} which predicts the input and avoids information loss. The family of autoencoders \cite{Vincent2008,HeCXLDG22} provide an alternative information-preserving framework for self-supervised learning using a reconstruction loss. The common drawback of the above-mentioned methods is the lack of structure in representations, which proves key to their expressivity and generalization.

\textbf{Structured and equivariant representations} Learning structured representations is one efficient strategy to maintain information in the data, since the latent variables can be organized in a compact way. In the unsupervised learning domain, existing works like \cite{isa_vae} have extensively explored structured latent priors for the Variational Autoencoder (VAE) \cite{Kingma2014}, while the recent Topographic VAE \cite{tvae} aims to induce topographic organization of the observed set of transformations. The idea of structured representations has also been connected to unsupervised learning of disentangled representations \cite{betavae,kumar2018variational}. Another closely related line of work focuses on learning equivariance \cite{gcnn, sesn, arblie, qtae, offseteq} as a more general form of representation structure. For example, \cite{sesn} propose to use a basis of transformed filters to learn equivariant features, which generally leads to improved model robustness and data efficiency.

\textbf{MSSL} based on invariance learning has seen great success, and can be broadly grouped into two categories of methods: contrastive learning between augmented views of different data \cite{simclr, moco, swav}, and non-contrastive methods by only comparing the same data views \cite{byol, btwins}. 
\todo{Dan to add comment about https://arxiv.org/abs/2102.08850 and https://arxiv.org/abs/2005.10242}
%To our knowledge, the structure of MSSL representations with respect to different transformations is barely studied in the literature.
This hinders the understanding of the underlying properties and generalization mechanisms of MSSL. Few exceptions exist, including the AugSelf \cite{augself} and equivariant method ESSL \cite{essl}, both of which are predictive of transformation parameters. However, these methods cannot induce structured representations. NPTN \cite{nptn}, on the other hand, learns structured representations from a basis of learned filters, but loses the equivariance property. Here we propose a new method to learn both structured and equivariant representations, with interesting observations on these properties.

% \paragraph{Structured representations}
% Many reasoning systems, including the human brain, show topographic organization \cite{wiringtopo} as a mechanism to maximize performance/resources trade-off. The underlying idea is that spatially nearby neurons should behave similarly (correlated). In the deep learning field, several works have attempted at learning organized representations \cite{tvae}. 
% ...
